QEVSEC: Quick Electric Vehicle SEcure Charging via Dynamic Wireless Power Transfer

Dynamic Wireless Power Transfer (DWPT) can be used for on-demand recharging of Electric Vehicles (EV) while driving. However, DWPT raises numerous security and privacy concerns. Recently, researchers demonstrated that DWPT systems are vulnerable to adversarial attacks. In an EV charging scenario, an attacker can prevent the authorized customer from charging, obtain a free charge by billing a victim user and track a target vehicle. State-of-the-art authentication schemes relying on centralized solutions are either vulnerable to various attacks or have high computational complexity, making them unsuitable for a dynamic scenario. In this paper, we propose Quick Electric Vehicle SEcure Charging (QEVSEC), a novel, secure, and efficient authentication protocol for the dynamic charging of EVs. Our idea for QEVSEC originates from multiple vulnerabilities we found in the state-of-the-art protocol that allows tracking of user activity and is susceptible to replay attacks. Based on these observations, the proposed protocol solves these issues and achieves lower computational complexity by using only primitive cryptographic operations in a very short message exchange. QEVSEC provides scalability and a reduced cost in each iteration, thus lowering the impact on the power needed from the grid.

==> tables/table_communication_comparison.tex <==
\begin{table}[!b]
\begin{center}
    \caption{Communication cost comparison, showing the total number of bytes used for the protocol. Our approach requires more bytes at the beginning, but then it is lighter than \cite{hussain2015} thanks to the hash-chain-only authentication with CPs.}
    \begin{tabular}{|l|l|l|}
        \textbf{} & \textbf{Our Solution}  & \textbf{\textit{Hussain et al.}\cite{hussain2015}}\\
        Pre-authentication & $32 \times 3$ B  & \textemdash \\
        Auth OBU & $32 \times 5$ B  & $32 \times 5$ B \\
        Auth CP / CSPA & $32 + 64$ B & $32 \times 4$ B \\
        Hash-chain & $32$ B per CP & \textemdash \\
        Total cost & $352 + 32 \times n$ B & $288 \times n$ B \\
    \end{tabular}
    \label{table:comparison-comm}
\end{center}
\end{table}

==> tables/table_comparison_computation.tex <==
\begin{table*}[!h]
\begin{center}
    \caption{Computational cost comparison. We show that our approach requires only a very slightly higher time during the beginning part comparing only one CP, but then it grows linearly with a very fast hash operation.}
    \begin{tabular}{|p{2.5cm}|p{3.25cm}|p{3.25cm}|p{3.25cm}|p{3.25cm}|}
        \hline
        & \textbf{Auth OBU}  & \textbf{Auth CP/CSPA/CMC} & \textbf{Hash-chain} & \textbf{Total time}\\
        \hline
        \textbf{Hussain \textit{et al.}} \cite{hussain2015} & 6$T_{h}$ + 6$T_{XOR}$ = 1.62 ms  &  7$T_{h}$ + 6$T_{XOR}$ = 1.89 ms & \textemdash & $3.51 \times n$ ms \\
        \hline
        \textbf{Rabieh \textit{et al.}} \cite{rabieh} & 4$T_{exp}$ + 4$T_{ecm}$ + 2$T_{ver}$ + $T_{sig}$ + $T_{h}$ = 10.01 ms & 2$T_{pair}$ + 4$T_{ecm}$ + 4$T_{exp}$ + $T_{sig}$ + $T_{ver}$ = 10.01 ms & $n \times 0.27$ ms & $20.02 +  T_{Hash-chain}$ ms \\
        \hline
        \textbf{Zhao \textit{et al.}} \cite{zhao} & 2$T_{sig}$ + 2$T_{ver}$ + $T_{h}$ = 5.15 ms  & $T_{sig}$ + 2$T_{ver}$ = 3.89 ms  & $ n \times 0.27 + n \times (T_{sig} + T_{ver})$ ms & $9.04 + T_{Hash-chain}$ ms \\
        \hline
        \textbf{QEVSEC} &\textbf{6$\mathbf{T_h}$ + 5$\mathbf{T_{XOR}}$ + $\mathbf{T_{exp}}$ = 1.73 ms} & 
        \textbf{8$\mathbf{T_{h}}$ + 5$\mathbf{T_{XOR}}$ + $\mathbf{T_{exp}}$ = 2.27 ms} & \textbf{$\mathbf{n \times 0.27}$} & \textbf{$\mathbf{4.00 + }$  $\mathbf{T_{Hash-chain}}$ ms} \\
        \hline
    \end{tabular}
    \label{table:comparison}
\end{center}
\end{table*}

==> tables/table_computation_cost.tex <==
\begin{table}[!h]
    \begin{center}
        \caption{Cryptographic primitive execution time.}
        \begin{tabular}{|p{1.5cm}|p{1.75cm}|}
            \hline  
            \textbf{Primitive} & \textbf{Average Time (ms)} \\ 
            \hline
            $T_{exp}$ & 0.110 \\ 
            \hline
            $T_{pair}$ & 0.884 \\ 
            \hline
            $T_{h}$ & 0.27  \\
            \hline
            $T_{ecm}$ & 1.352 \\
            \hline
            $T_{ver}$  & 1.449 \\ 
            \hline
            $T_{sig}$  & 0.992 \\
            \hline
        \end{tabular}
        \label{table:computational_cost}
    \end{center}
\end{table}

